Locally Fair Partitioning

We model the societal task of redistricting political districts as a partitioning problem: Given a set of $n$ points in the plane, each belonging to one of two parties, and a parameter $k$, our goal is to compute a partition $\Pi$ of the plane into regions so that each region contains roughly $\sigma = n/k$ points. $\Pi$ should satisfy a notion of ''local'' fairness, which is related to the notion of core, a well-studied concept in cooperative game theory. A region is associated with the majority party in that region, and a point is unhappy in $\Pi$ if it belongs to the minority party. A group $D$ of roughly $\sigma$ contiguous points is called a deviating group with respect to $\Pi$ if majority of points in $D$ are unhappy in $\Pi$. The partition $\Pi$ is locally fair if there is no deviating group with respect to $\Pi$. This paper focuses on a restricted case when points lie in $1$D. The problem is non-trivial even in this case. We consider both adversarial and ''beyond worst-case" settings for this problem. For the former, we characterize the input parameters for which a locally fair partition always exists; we also show that a locally fair partition may not exist for certain parameters. We then consider input models where there are ''runs'' of red and blue points. For such clustered inputs, we show that a locally fair partition may not exist for certain values of $\sigma$, but an approximate locally fair partition exists if we allow some regions to have smaller sizes. We finally present a polynomial-time algorithm for computing a locally fair partition if one exists.

==> fig/graph_relaxed.tex <==
\begin{figure}[ht]
\centering
\begin{tikzpicture}[scale=0.75]
\label{grph:relaxed}
\begin{axis}[
        xlabel=$\eps$,
        ylabel=$\beta$,
        xmin=0,xmax=1/2,
        ymin=0,ymax=1.7]
%lower & upper bounds
\addplot[domain=0:1/2, color=black,name path=upper]{1+x};
\addplot[domain=0:1/2, color=black,name path=lower]{(1-x)/2};
%
\addplot[domain=0:1/2, color=black, dotted, name path=B]{1};
% \addplot[domain=1/2:1/2, color=black, dotted, name path=C]{1/2+x};
\addplot[domain=0:1/2, color=black, dotted, name path=D]{1};
\addplot[domain=0    : 1/5,  color=black, dotted, name path=D2a]{(2*(1-x))/2};
\addplot[domain=1/5  : 2/6,  color=black, dotted, name path=D2b]{((3*x)+1)/2};
\addplot[domain=2/6  : 3/7,  color=black, dotted, name path=D3a]{(3*(1-x))/2};
\addplot[domain=3/7  : 4/8,  color=black, dotted, name path=D3b]{(4*x)/2};
% \addplot[domain=4/8  : 5/9,  color=black, dotted, name path=D4a]{(4*(1-x))/2};
% \addplot[domain=5/9  : 6/10, color=black, dotted, name path=D4b]{(5*x-1)  /2};
% \addplot[domain=6/10 : 7/11, color=black, dotted, name path=D5a]{(5*(1-x))/2};
% \addplot[domain=7/11 : 8/12, color=black, dotted, name path=D5b]{(6*x-2)  /2};
%..
\addplot[domain=0:1/2, color=black, dotted, name path=m10]{1-x};
% \addplot[domain=1/2:1, color=black, dotted, name path=ext10]{x};
%Shading positive
%\addplot[blue!20] fill between[of=D and D2a];
\addplot[blue!20] fill between[of=D and D2b];
\addplot[blue!20] fill between[of=D and D3a];
%\addplot[blue!20] fill between[of=D and D3b];
%\addplot[blue!20] fill between[of=upper and D4a];
%\addplot[blue!20] fill between[of=upper and D5a];
\addplot[blue!20] fill between[of=upper and D];
%\addplot[blue!20] fill between[of=upper and B];
%other known values..
% \draw [blue, ultra thick] (1,0) -- (1,1);
%negative results
\addplot[red!20] fill between[of=lower and m10];
% \addplot[red!20] fill between[of=lower and ext10]; 
%text...
% \node[] at (axis cs: 0.75,0.9) {...};
\end{axis}
\end{tikzpicture}
\caption{For blue $(\eps, \beta)$, a locally fair solution always exists. For red $(\eps, \beta)$, there exists an instance with no locally fair solution.}
\label{fig:characterization}
\end{figure}
